DDI-CoCo: A Dataset For Understanding The Effect Of Color Contrast In Machine-Assisted Skin Disease Detection

Skin tone as a demographic bias and inconsistent human labeling poses challenges in dermatology AI. We take another angle to investigate color contrast's impact, beyond skin tones, on malignancy detection in skin disease datasets: We hypothesize that in addition to skin tones, the color difference between the lesion area and skin also plays a role in malignancy detection performance of dermatology AI models. To study this, we first propose a robust labeling method to quantify color contrast scores of each image and validate our method by showing small labeling variations. More importantly, applying our method to \textit{the only} diverse-skin tone and pathologically-confirmed skin disease dataset DDI, yields \textbf{DDI-CoCo Dataset}, and we observe a performance gap between the high and low color difference groups. This disparity remains consistent across various state-of-the-art (SoTA) image classification models, which supports our hypothesis. Furthermore, we study the interaction between skin tone and color difference effects and suggest that color difference can be an additional reason behind model performance bias between skin tones. Our work provides a complementary angle to dermatology AI for improving skin disease detection.

==> fig_DA_contrast.tex <==
\begin{figure*}[htb!]
    \begin{minipage}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/TRANS_ISIC2019_DA_TEST_ddi_efficientnet_contrast.jpeg}
         \centerline{(a)}
     \end{minipage}\hfill
    \begin{minipage}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/TRANS_ISIC2019_DA_TEST_ddi_swin_contrast.jpeg}
         \centerline{(b)}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/FINETUNE_ddi_DA_TEST_ddi_efficientnet_contrast.jpeg}
         \centerline{(c)}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/FINETUNE_ddi_DA_TEST_ddi_swin_contrast.jpeg}
         \centerline{(d)}
     \end{minipage}
    \caption{\textbf{Data augmentation results on contrast groups.} (a)(b) Objective 1: we train models on ISIC 2019 with different DA methods, and evaluate on DDI-CoCo. (c)(d) Objective 2: we train models on ISIC2 2019, fine-tune on 80\% of DDI-CoCo with different DA methods, and evaluate on 20\% of DDI-CoCo. We observe that RandAugment (RA) can mitigate the performance gap between contrast groups in objective 1. However, we do not observe RA benefit in other cases, the same goes for Cutmix and Mixup. Detailed discussion is in Sec.~\ref{sec:DA}.}
    \label{fig:DA_contrast}
    % \vspace{-5mm}
\end{figure*}

==> fig_auc_by_skintone.tex <==
\begin{figure}
    \begin{minipage}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_inception.png}
         \caption{Inception V3}
     \end{minipage}\hfill
    \begin{minipage}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_efficient.png}
         \caption{EfficientNet V2}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_swin.png}
         \caption{Swin Transformer}
     \end{minipage}\hfill
     
     % \begin{minipage}[b]{0.48\textwidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/auc_by_skintone_wideresnet.png}
     %     \caption{WideResnet101}
     % \end{minipage}
    \caption{\textbf{AUC by Skin Tones.} }
    \label{fig:auc_by_skintone}
\end{figure}

==> fig_barplot.tex <==
\begin{figure}
    \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bar_efficient.png}
         \caption{EfficientNetV2}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bar_swin.png}
         \caption{Swin Transformer}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bar_inception.png}
         \caption{Inception V3}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bar_wideresnet_v1.png}
         \caption{WideResnet101}
     \end{minipage}
    \caption{Caption}
    \label{fig:barplot_by_contrast}
\end{figure}

==> fig_contrast_std.tex <==
\begin{figure}
    \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/coy_skintone_efficient.png}
         \caption{EfficientNetV2}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_swin.png}
         \caption{Swin Transformer}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_inception.png}
         \caption{Inception V3}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/auc_by_skintone_wideresnet.png}
         \caption{WideResnet101}
     \end{minipage}
    \caption{Caption}
    \label{fig:label_dist}
\end{figure}

==> fig_label_dist.tex <==
\begin{figure}
    \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/contrast_dist.png}
         \caption{black}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/contrast_std.png}
         \caption{black}
     \end{minipage}
    \caption{Caption}
    \label{fig:label_dist}
\end{figure}

==> fig_roc_architectures.tex <==
\begin{figure}
    \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_efficient.png}
         \caption{EfficientNetV2}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_swin.png}
         \caption{Swin Transformer}
     \end{minipage}
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_wideresnet.png}
         \caption{WideResnet101}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_inception.png}
         \caption{Inception V3}
     \end{minipage}
    \caption{\textbf{ROC curve by models.} Transformer model has a better FST V-VI performance, which is contrary to CNN based models. This validates our assumption that model architecture will play a certain role.}
    \label{fig:label_dist}
\end{figure}

==> fig_roc_skin.tex <==
\begin{figure}[t]
    \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_skin12.png}
         \caption{FST I-II}
     \end{minipage}\hfill
     % \begin{minipage}[b]{0.45\textwidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/roc_skin34.png}
     %     \caption{black}
     % \end{minipage}
     \begin{minipage}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/roc_skin56.png}
         \caption{FST V-VI}
     \end{minipage}
   
    \caption{advaned pre-training on wideresnet101 (purple) does not show better result than standard wideresnet101 (red)}
    \label{fig:label_dist}
\end{figure}

==> fig_violin_rgb.tex <==
\begin{figure}[t]
     \centering
         \includegraphics[width=0.5\linewidth]{figures/violin_rgb.png}    
    \caption{\textbf{Background RGB values by skin tones.} We observe that dark skin tone has smaller RGB values, showing our human-judgement-agnostic method correlate with the actual outcome. }
    \label{fig:violin_rgb}
\end{figure}

==> tab_DA_overall_auc.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{lcccc}\toprule
      DA method   &  Objective1-EfficientNet & Objective1-SwinV2 & Objective2-EfficientNet & Objective2-SwinV2\\\midrule
    No DA & 0.630 & 0.686 & 0.805 & 0.826\\
    RA \cite{cubuk2020randaugment} & 0.629 & 0.680 & 0.803 & 0.806\\
    Mixup \cite{zhang2017mixup}& 0.620 & 0.696 & 0.801 & 0.805\\
    Cutmix \cite{yun2019cutmix}& 0.626 & 0.708 & 0.810 & 0.796\\\bottomrule
    \end{tabular}
    \caption{\textbf{Average AUC with and without data augmentations.} On both our experimental objectives (Sec.~\ref{sec:methods}), we do not see obvious benefits of using DAs (improvements only show in three cases).}
    \label{tab:da_overall_auc}
\end{table*}

==> tab_model_size.tex <==
\begin{table}[]
    \begin{subtable}[h]{0.45\textwidth}
    \centering
    \caption{\textbf{Number of images by contrast.}\ming{add filtered back and remove III-IV?}}
    \begin{tabular}{lc}\toprule
      Architecture   &  \#parameters \\\midrule
    InceptionV3 & 27.2M \\
    EfficientNet V2 & 21.5M \\
    Swin Transformer & 87.9M \bottomrule
    \end{tabular}
    \label{tab:contrast}
\end{table}

==> tab_setups.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lcc}\toprule
       & Training   &  Fine-tuning \\\midrule
    Optimizer & Adam & Adam\\
    Epochs & 60 & 50 \\
    Batch Size & 128 & 64\\
    LR & 0.0001 & 0.0001 \\\bottomrule
    \end{tabular}
    \caption{\textbf{Training \& fine-tuning hyperparameters.} We emulate the fine-tuning process in \cite{dosovitskiy2020vit}. We choose hyperparameters based on the dataset sizes --- for ISIC 2019, we train about 10k steps; for DDI we fine-tune about 500 steps.}
    \label{tab:appendix_setups}
\end{table}
